HEAP -- The autonomous walking excavator

The demand and the potential for automation in the construction sector is unmatched, particularly for increasing environmental sustainability, improving worker safety and reducing labor shortages. We have developed an autonomous walking excavator - based one of the most versatile machines found on construction sites - as one way to begin fulfilling this potential. This article describes the process of converting an off-the-shelf construction machine into an autonomous robotic system. First we outline the necessary sensing equipment for full autonomy and the novel actuation of the legs, and compare three different complementary actuation principles for the excavator's arm. Second, we solve the state estimation problem for a general wheeled-legged robot. Beside kinematic measurements, it includes GNSS-RTK, to absolutely reference the machine on a construction site. Third, we developed individual controllers for driving, chassis balancing and arm motions allowing for fully autonomous operation. Lastly, we highlight the machine's potential in four different real-world applications, e.g. autonomous trench digging, autonomous assembly of dry stone walls, autonomous forestry work and semi-autonomous teleoperation. On top, we also share some development insights and possible future research directions.

==> state_estimation_long.tex <==
\section{State Estimation}\label{sec:state_estimation}

The state estimator of HEAP is implemented using the two-state implicit filter (TSIF) of Bloesch et al. \cite{Bloesch_2018_tsif}. TSIF is a purely residual based filter and therefore facilitates modularity and allows for a larger spectrum of models to be incorporated in the estimation compared to a more conventional Extended Kalman Filter. 

The position measurement of the cabin turn joint, connecting the upper machine to the chassis is realized with two inductive sensors that detect passing gear teeth. An additional inductive sensor corrects potential errors of this incremental measurement when passing zero. Due to the low number of teeth in the large internal ring gear (98 teeth in total), an angular resolution of only 0.92$^\circ$ can be achieve. Thus fusing the chassis IMU with the GNSS measurement of the cabin would lead to a high error. Instead, GNSS measurements are fused with the cabin IMU and the state will be estimated in the cabin frame $C$. The chassis and cabin IMU are used to augment the cabin turn angle measurement in a complementary filter. The cabin turn angular velocity $\dot{\psi}$ is estimated as the difference of the angular velocities of the cabin IMU ($C$ frame) and the chassis IMU ($B$ frame) in joint direction $z$ as
\begin{equation}
    \dot{\psi}' = {\tilde{\omega}_{BCz}} = {\tilde{\omega}_{ICz}} - {\tilde{\omega}_{IBz}} .
\end{equation}
The low quality turn angle measurement $\tilde{\psi}$ is augmented with the measured turn angular velocity in a complementary filter with the weighting constant $\alpha$ to compute the turn angle estimate $\psi'$ as follows
\begin{equation}
    \psi' = \alpha \tilde{\psi} + (1-\alpha)(\psi + \Delta t \dot{\psi}).
\end{equation}
The full robot state can then be computed using four residuals, namely IMU prediction, GNSS update, rolling prediction and legged odometry update, from two GNSS measurements, cabin IMU and all joint sensors.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{IMU Prediction} \label{sec:imu}
Using measurements from the cabin IMU one can formulate a straight forward prediction of the state
\begin{equation}
    x_{\text{IMU}} = \left( {_{I}r}_{IC},\ \Phi_{CI},\ {_{I}v}_{IC},\ {{_C}b}_{f},\ {{_C}b}_{\omega} \right)
\end{equation}
where $_{I}{r}_{IC} \in \mathbb{R}^3$ represents the position of the cabin frame $C$ relative to the inertial frame $I$, which together with the orientation $\Phi_{CI}$ constitutes the pose of the system. The orientation is represented here by $\Phi_{CI}$. It is used interchangeably as an abstract orientation in $SO(3)$ as well as the corresponding rotation mapping $\Phi_{CI}: \mathbb{R}^3 \rightarrow \mathbb{R}^3$ such that $\Phi_{CI}({_{I}\eta})={_{C}\eta}$ for all vectors $\eta$ in 3 dimensional space. Throughout this text, left subscripts will denote the frame in which a vector is expressed. The state also includes the linear velocity $_{I}{v}_{IC} \in \mathbb{R}^3$ of the cabin relative to the inertial frame and bias vectors $_{C}b_f$ and $_{C}b_\omega \in \mathbb{R}^3$ for linear acceleration and angular velocity respectively to model drift in the IMU. Angular velocity is excluded from the state since it is measured directly.\\

The kinematics of the cabin frame origin in continuous time are
\begin{align}
    _{I}\dot{r}_{IC}&={_{I}v}_{IC} \label{posode} \\
    \dot{\Phi}_{CI}&=-_{C}\omega_{IC}\\
    _{I}\dot{v}_{IC}&={_{I}a}_{IC}=\Phi_{CI}^{-1}({_{C}f_{IC}})+{_{I}g}
\end{align}
This introduces $_{C}\omega_{IC} \in \mathbb{R}^3$ for the angular velocity of the cabin frame and the linear acceleration $_{I}a_{IC}$ which splits into the gravity vector $_{I}g$ and the proper acceleration ${_{C}f_{IC}}$ as measured by the IMU. See \cite{Bloesch_2016_primer} for references on the calculus of 3D orientations $\Phi$. There is stationary white noise $w_f$ and $w_\omega$ on the IMU measurements, denoted $\tilde{f}_{IC}$ and $\tilde{\omega}_{IC}$. Adding the biases from the filter state, the IMU measurements write
\begin{align}
    {_{C}\tilde{f}}_{IC}&={_{C}f}_{IC}+{_{C}b_{f}}+{_{C}w_f}\\
    {_{C}\tilde{\omega}}_{IC}&={_{C}\omega}_{IC}+{_{C}b_{\omega}}+{_{C}w_\omega}
\end{align}
which allows to integrate the measurements into the kinematics, yielding
\begin{align}
    _{I}\dot{v}_{IC}&= \Phi_{CI}^{-1}({_{C}\tilde{f}}_{IC} - {_{C}b_{f}} - {_{C}w_f}) +{_{I}g}\\
    \dot{\Phi}_{CI}&=-({_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}-{_{C}w_\omega})
\end{align}
Using these expressions as well as equation \ref{posode} for the linear velocity, an Euler forward discretization of the kinematics by a time step $\Delta t$ results in the first part of the prediction equations using IMU measurements
\begin{align}
    {_{I}r}_{IC}' &= {_{I}r}_{IC} + \Delta t\left[ {_{I}v}_{IC} +\frac{{{_I}\bar{w}_v}}{\sqrt{\Delta t}} \right]\label{pospred} \\
    \begin{split}
            {_{I}v}_{IC}' &= \\ &{_{I}v}_{IC} + \Delta t\left[ \Phi_{CI}^{-1}\left({_{C}\tilde{f}}_{IC} - {_{C}b_{f}} - \frac{{_{C}\bar{w}_f}}{\sqrt{\Delta t}}\right) +{_{I}g} \right]
    \end{split}\\
    \Phi_{CI}' &= \Phi_{CI} \boxplus \left[ -\Delta t\left({_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}-\frac{{_{C}\bar{w}_\omega}}{\sqrt{\Delta t}}\right)\right]\label{orpred}
\end{align}
These equations introduce the notational shortcut of referring to current states with primes - e.g. ${_{I}r}_{IC}'$ - while past states are unprimed. The ${_F}w_j$ have been discretized using zero-order-hold equivalence as $\frac{{_{F}\bar{w}_j}}{\sqrt{\Delta t}}$ for $F \in \left\{ I,\ C \right\}$, $j \in \left\{ v,\ f,\ \omega \right\}$, where the ${_{F}\bar{w}_j}$ are discrete time gaussian noise distributed ${_{F}\bar{w}_j} \sim \mathcal{N}(0,Q_j)$ at each iteration. The $Q_j \in \mathbb{R}^{3\times3}$ are tuning parameters of the estimation algorithm, capturing the properties of the IMU system as well as serving as weighting factors between different residuals operating on the same states (ignoring the weighting aspect and minding the $\frac{1}{\sqrt{\Delta t}}$ factor in the noise discretization, the $Q_j$ are the spectral densities of the continuous-time white noise). The position prediction Equation \ref{pospred} introduces such a weighting factor to possibly weaken the influence of the IMU on position estimates. 

Also part of the IMU residual is the prediction of the IMU biases. Modelling the biases as Brownian Motions in a standard engineering way lets one write their derivatives as
\begin{equation}
    {_C\dot{b}_i} = {_C{w}_{b,i}} ,\, i \in \left \{ f,\ \omega \right \}
\end{equation}
with white noise vectors ${_C{w}_{b,i}}$. Using the same discretization procedure as above results in the prediction equations for the IMU biases
\begin{equation}\label{bpred}
    {_C{b}'_{i}} = {_C{b}_{i}} + \sqrt{\Delta t} {{_C}\bar{w}}_{b,i}\
\end{equation}
Again, the time-discrete noise vectors are distributed ${{_C}\bar{w}}_{b,i} \sim \mathcal{N}(0,Q_{b,i})$.\\

Equations \ref{pospred} to \ref{orpred} together with the two equations represented by \ref{bpred} make up the full prediction equations for the IMU residual.\\

Having defined the IMU prediction residual with the prediction equations above, one can now calculate the Jacobians needed to apply them in the TSIF equations. The following is a list of the nonzero $3\times3$ blocks in the prediction Jacobians with respect to the state (all Jacobians throughout this chapter are evaluated at zero noise). The position Jacobians write
\begin{align}
    \frac{\partial {_{I}r}_{IC}'}{\partial {_{I}r}_{IC}} = \mathbb{I}, &&
    \frac{\partial {_{I}r}_{IC}'}{\partial {_{I}v}_{IC}} = \Delta t\ \mathbb{I}
\end{align}
with $\mathbb{I}$ the identity matrix. For the velocity Jacobians one obtains
\begin{align}
    \frac{\partial {_{I}v}_{IC}'}{\partial {_{I}v}_{IC}} = \mathbb{I}, &&
    \frac{\partial {_{I}v}_{IC}'}{\partial {_{C}b}_{\omega}} = -\Delta t\  R(\Phi_{CI})^{T}
\end{align}
\begin{equation}
    \frac{\partial {_{I}v}_{IC}'}{\partial {\Phi}_{CI}} = \Delta t\  R(\Phi_{CI})^{T} \left({_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}\right)^{\times}
\end{equation}
Where $R$ is the mapping from $SO(3)$ (or the rotation quaternions) to rotation Matrices and $_{F}\eta^{\times}$ denotes the skew symmetric matrix obtained from a vector $_{F}\eta \in \mathbb{R}^3$ represented in some frame $F$. The bias Jacobians only contain
\begin{align}
    \frac{\partial {_C{b}'_{b,i}}}{{_C{b}_{b,i}}} = \mathbb{I}
\end{align}
The orientation Jacobians use the $\Gamma$ matrix representing the Jacobian of the exponential map for the quaternion representation \cite{Bloesch_2016_primer}
\begin{align}\label{imurotjacs}
    \frac{\partial {\Phi}_{CI}'}{\partial {\Phi}_{CI}} &= R\left(exp\left(-\Delta t \left[ {_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}\right]\right)\right)\\
    \frac{\partial {\Phi}_{CI}'}{\partial {_{C}b_{\omega}}} &= \Delta t \  \Gamma \left(-\Delta t \left[ {_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}\right]\right)
\end{align}
Finally, the last objects needed for the implementation of the residual are the prediction Jacobians with respect to the noise
\begin{align}
    \frac{\partial {_{I}r}_{IC}'}{\partial {_{I}\bar{w}_v}} &= \sqrt{\Delta t}\ \mathbb{I}\\ 
    \frac{\partial {_{I}v}_{IC}'}{\partial {_{C}\bar{w}_f}} &= -\sqrt{\Delta t}\  R(\Phi_{CI})^{T}\\
    \frac{\partial {\Phi}_{CI}'}{\partial {_{C}\bar{w}_\omega}} &= \sqrt{\Delta t} \  \Gamma\left(-\Delta t \left[ {_{C}\tilde{\omega}}_{IC}-{_{C}b_{\omega}}\right]\right)\\ 
    \frac{\partial {_C{b}'_{b,i}}}{\partial {{_C}\bar{w}}_{b,i}} &= \sqrt{\Delta t}\ \mathbb{I}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{GNSS Update} \label{sec:gnss}
 The GNSS sensors provide absolute position measurements that allow to locate the cabin within the inertial frame. The innovation equation is again a comparison of the measurement and the sensor location computed from the estimator state. The state for this residual is
\begin{equation}
x'_{GNSS} = \left({_{I}r'_{IC}},\ \Phi'_{CI} \right).
\end{equation}
The innovation equation for the two sensors $k=\{1,2\}$ is
\begin{equation} \label{gpsinn}
y_{\xi_k} = {_{I}\tilde{\xi_k}} - {_{I}r'_{IC}} - \Phi_{CI}'^{-1}({_{C}l_{C\xi_k}}) + {_{I}\bar{w}_{\xi_k}}.
\end{equation}

The GNSS position measurement in inertial coordinates is represented by ${_{I}\tilde{\xi_k}}$. The second and third term in equation \ref{gpsinn} are a homogeneous transformation from the GNSS sensor location in the cabin frame $C$, which is denoted ${_{C}l_{C\xi}}$, into the inertial frame. The GNSS measurement noise is again distributed as ${_{I}\bar{w}_{\xi_k}} \sim \mathcal{N}(0,Q_{\xi_k})$.

The results for the innovation Jacobian blocks with respect to the state are
\begin{align}
\frac{\partial y_{\xi_k}}{\partial {_{I}r'_{IC}}} = -\mathbb{I}, &&
\frac{\partial y_{\xi_k}}{\partial \Phi'_{CI}} = -R(\Phi'_{CI})^{T} \left[{_{C}l_{C\xi_k}}\right]^{\times}
\end{align}
while the innovation Jacobian with respect to the noise is
\begin{align}
\frac{\partial y_{\xi_k}}{\partial {_{I}\bar{w}_{\xi_k}}} &= \mathbb{I}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rolling Prediction} \label{sec:roll}

To use the contact points of the M545's four wheels as landmarks in the same way footholds were used on StarlETH, this residual implements a prediction of those contact points using measurements of the wheel speeds together with a kinematic model of the system to get wheel forward directions. This allows basic odometry for each contact point separately. In continuous time the kinematics for each contact point ${_{I}{p}_{i}} \in \mathbb{R}^3$, $i \in \left \{ rf,\ lf,\ lh,\ rh\right \}$ (i.e. right front, left front, left hind and right hind) write
\begin{align}\label{rollpred}
{_{I}\dot{p}_{i}} = \Phi_{BI}^{-1}( \rho \dot{\varphi}_i {_{B}{\bar{\nu}_i}} +{{_B}w}_{p,i})
\end{align}
There is white noise ${{_B}w}_{p,i}$ on the contact point velocity, which is treated in the same way as the IMU kinematics noise was. The wheel radii are assumed to be identical and represented by $\rho \in \mathbb{R}$, while $\dot{\varphi}_i \in \mathbb{R}$ denotes the $i$-th rotational wheel speed. Together with the wheel forward directions ${_{B}{\bar{\nu}_i}} \in \mathbb{R}^3$ they make up the velocity of the contact points.\\

%The ${_{B}{\bar{\nu}_i}}$ are obtained from a kinematic model of the M545, which is configured with the pose estimates from the GIF and joint position measurements. The model actually outputs unit vectors ${_{B}{\nu_i}}$ which are obtained in the following way. Each wheel is connected to its respective leg by a knuckle link as illustrated in figure \ref{fig:knuckles}. These screengrabs of the M545 Gazebo simulation show the inertial world frame $I$ together with the body-fixed frame of the left front knuckle link for 2 different stances of the system. It is immediately apparent that the orientation of the knuckle is affected by the stance. The wheel forward direction provided by the model now corresponds to the red $x$-axis of the knuckle frame, which may point into or out of the ground plane if the M545's joints deviate from their default configuration. This in turn makes the contact points dive into or lift off of the terrain, thus corrupting the odometry.

The ${_{B}{\nu_i}}$ are projected into a plane defined by a terrain normal vector $n \in \mathbb{R}^3$ to obtain ${_{B}{\bar{\nu}_i}}$ as
\begin{equation}\label{proj}
{_{B}{\bar{\nu}_i}} = {_{B}{\nu_i}} - {_{B}{\nu_i}}^{T} \Phi_{BI}({_{I}n})\ \Phi_{BI}({_{I}n})
\end{equation}
The terrain normal is assumed to be known for this, which was the case for the simulated environment used during this work, but would make it necessary to utilize terrain estimation in more challenging terrain.

As in section \ref{sec:imu}, an Euler forward discretization of equation \ref{rollpred} now yields prediction equations for the contact points
\begin{align}
{_{I}p'_{i}} = {_{I}p_{i}} + \Delta t \ \Phi_{BI}^{-1}\left( \rho\dot{\tilde{\varphi}}_i {_{B}{\bar{\nu}_i}} +\frac{{_B}\bar{w}_{p,i}}{\sqrt{\Delta t}}\right)
\end{align}
with the discrete-time noise again distributed ${{_B}\bar{w}}_{p,i} \sim \mathcal{N}(0,Q_{p,i})$ and $\dot{\tilde{\varphi}}_i$ representing - by some abuse of notation - a discrete-time measurement of the wheel speed $\dot{\varphi}_i$. At this point, combining equation \ref{proj} with the prediction results in the four innovation equations of the Rolling Prediction residual
\begin{multline}\label{rollinn}
y_{p,i} = {_{I}p_{i}} + \Delta t \ \Phi_{BI}^{-1}\left( \rho\dot{\tilde{\varphi}}_i {_{B}{\nu_i}} +\frac{{_B}\bar{w}_{p,i}}{\sqrt{\Delta t}}\right) \\ - \Delta t \rho\dot{\tilde{\varphi}}_i \ {{_I}n} {_{B}{\nu_i}}^{T} \ \Phi_{BI}({{_I}n}) - {_{I}p'_{i}} 
\end{multline}
%From this one can read off the states on which the Rolling Prediction operates, namely
%\begin{equation}
%x_{Roll} = \left(\Phi_{BI},\ {_{I}p_{i}} \right)
%\end{equation}
%Note that the current orientation does not appear in equation \ref{rollinn}, which makes it more precise to say that the Rolling Prediction connects previous contact points and orientation $\left(\Phi_{BI},\ {_{I}p_{i}} \right)$ with the current contact points ${_{I}p'_{i}}$.\\

What remains to do is the calculation of the innovation Jacobians. The Jacobian blocks with respect to the current state simply are
\begin{align}
\frac{\partial y_{p,i}}{\partial {_{I}p'_{i}}} &= -\Delta t\ \mathbb{I}
\end{align}
Similarly, the Jacobian blocks with respect to the previous state write
\begin{multline}
\frac{\partial y_{p,i}}{\partial {\Phi_{BI}}} = \Delta t\ C(\Phi_{BI})^{T} (\rho\dot{\tilde{\varphi}}_i {_{B}{\nu_i}})^{\times} \\ -\Delta t \rho\dot{\tilde{\varphi}}_i \ {{_I}n} {_{B}\nu_i}^{T}\ C(\Phi_{BI})\ {{_I}n}^{\times}
\end{multline}
\begin{equation}
\frac{\partial y_{p,i}}{\partial {_{I}p_{i}}} = \Delta t\ \mathbb{I}
\end{equation}
And the innovation Jacobian with respect to the noise is
\begin{align}
\frac{\partial y_{p,i}}{\partial {_{B}\bar{w}_{p,i}}} &= \sqrt{\Delta t}\ C(\Phi_{BI})^{T}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Legged Odometry Update} \label{sec:kin}

To complete the IMU and kinematics fusion strategy from \cite{imulegkin}, the contact point landmarks predicted by the Rolling Prediction are now used to locate the M545's base within the map composed of the four contact points. Again $i \in \left \{ rf,\ lf,\ lh,\ rh\right \}$ indexes the four legs. The innovation equations for this residual are a straight forward comparison of the contact points kept in the filter state on one hand, and the same contact points computed from measurements of the joint positions on the other. In this way, the residual updates both the pose and contact points simultaneously by minimizing the discrepancy between the current filter state and the measured configuration of the legs. The necessary state for this is
\begin{equation}
x'_{Roll} = \left({_{I}r'_{IB}},\ \Phi'_{BI},\ {_{I}p'_{i}} \right)
\end{equation}
where all of the states are current values. This corresponds to a standard measurement equation as used in an EKF setting. The actual measurements are the leg joint positions $\tilde{\alpha} \in \mathbb{R}^{12}$, which via the M545 kinematic model can be used to calculate vectors ${_{B}s_{i}(\tilde{\alpha})} \in \mathbb{R}^{3}$ from M545's base to the contact points. Similar to the way the wheel forward directions were calculated in section \ref{sec:roll} the contact points provided by the model are fixed with respect the last link of each leg.\\

Those vectors can also be calculated from $x'_{Roll}$ as $\Phi'_{BI}({_{I}p'_i} - {_{I}r'_{IB}})$, which results in the following innovation equation.
\begin{equation}
y_{s,i} = {_{B}s_{i}(\tilde{\alpha})} - \Phi'_{BI}({_{I}p'_i} - {_{I}r'_{IB}}) - {_{B}\bar{w}_{s,i}}
\end{equation}
Since the update is time-discrete, there is no need to worry about noise discretization and the measurement noise is again distributed as ${{_B}\bar{w}}_{s,i} \sim \mathcal{N}(0,Q_{s,i})$. The residual assumes constant wheel contact which is provided by the M545 controllers most of the time. However, there is the possibility of setting the entries of $Q_{s,i}$ very large in case the $i$-th leg lifts off, basically making the residual ignore its contact point as a landmark.\\

To follow \cite{imulegkin}, the $Q_{s,i}$ are calculated from the uncertainties in the joint position measurements as well as the kinematic model. Firstly, the ${_{B}s_{i}(\tilde{\alpha})}$ are modelled to be affected by additive gaussian noise with zero mean and covariances $R_{s,i}$. Secondly, there is uncertainty in the joint position measurements $\tilde{\alpha}$ themselves, which makes it necessary to propagate the covariance on the joint measurements through the model. Here there is need to take yet another step. Since joint positions on M545 are actually converted from piston displacements by a mapping $f_{\alpha\beta}: \mathbb{R}^{12} \rightarrow \mathbb{R}^{12}$ such that $\alpha = f_{\alpha\beta}(\beta)$ for the piston positions $\beta \in \mathbb{R}^{12}$, the $Q_{s,i}$ are obtained from
\begin{equation}
Q_{s,i} = R_{s,i} + J_{1} J_{2} R_{\beta} J_{2}^T J_{1}^T
\end{equation}
using the two Jacobians $J_{1} = \frac{\partial{_{B}s_{i}}}{\partial \alpha}$ and $J_{2} = \frac{\partial f_{\alpha\beta}}{\partial \beta}$. $R_\beta$ corresponds to the actual covariance of additive zero-mean gaussian noise on the piston measurements.\\

With the innovation equation in place, the Jacobians for this residual can be obtained. The blocks with respect to the states are
\begin{align}
    \frac{\partial y_{s,i}}{\partial {_{I}r}'_{IB}} = C(\Phi'_{BI}), && \frac{\partial y_{s,i}}{\partial {_{I}p'_i}} = -C(\Phi'_{BI})
\end{align}
\begin{equation}
    \frac{\partial y_{s,i}}{\partial \Phi'_{BI}} = \left[ C(\Phi'_{BI}) ({_{I}p'_i} - {_{I}r'_{IB}})\right]^{\times}
\end{equation}

And the entries of the innovation Jacobian with respect to the noise are calculated as
\begin{align}
\frac{\partial y_{s,i}}{\partial {_{B}\bar{w}_{s,i}}} &= -\mathbb{I}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Residual Setups}\label{sec:res_estimation}
%\begin{figure}[h!]
%    \centering
%    \subfloat[Estimated x,y and z-position of the base.]
%        {\includegraphics[width=\linewidth]{images/est_pos_crop.pdf}%
%        \label{fig:estimator_pos_results}}
%    \hfil
%    \subfloat[Estimated roll, pitch and yaw angles of the base.]
%        {\includegraphics[width=\linewidth]{images/est_orient_crop.pdf}%
%        \label{fig:estimator_orient_results}}
%    \caption{Position and orientation estimates of the IMU/GNSS setup (red), IMU/GNSS/Rolling Prediction/Legged Odometry setup (blue) are compared to ground truth (black) from simulation. The plots start with a freshly initialized estimator with unknown biases.}
%    \label{fig:estimator_results}
%\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/est_error_crop.pdf}
    \caption{The sum of squared errors in orientation is depicted in the upper plot and for the position in the lower plot. The estimator is initialized with unknown biases at time 0s and the machine stays stationary until time 12s, where it then starts to move the legs and drive. The IMU/GNSS approach in red shows higher initial errors, but outperforms the IMU/GNSS/Roll/Leg approach once the machine starts to move.}
    \label{fig:est_error}
\end{figure}

The estimator was tested in a Gazebo simulation environment, which provides accurate ground truth on all estimated states for evaluation. The individual sensors are simulated with realistic noise and drift parameters. First, IMU, GNSS, rolling and legged odometry residuals are combined in an attempt of feeding as much information to the estimator as possible. Figure \ref{fig:est_error} shows the estimated position and orientation of this setup in blue. It is apparent that the estimator does not perform well during yawing (driving a tight corner) and acceleration and deceleration. This is caused by the rolling and kinematics constraint that cannot account for wheel slip, estimation error of the ground plane and uncertainties about the ground contact point of the wheel (it's not a point foot as for legged robots). Thus, the second residual setup consists only of IMU and GNSS residuals. Its performance can be seen by the red line in Figure \ref{fig:est_error}. A large error is shown at the beginning after the estimator is initialized and disappears after the robot starts to move. The cause is that IMU biases cannot be estimated without motion in this setup. Once the biases have converged, the IMU/GNSS setup outperforms the full setup. 

The IMU/GNSS setup was deployed on the system. Which is not only motivated by the fact that rolling and kinematic constraints might not even improve the result in simulation, but also because on the real machine wheel speeds cannot be measured and wheels tend to slip even more. In future, visual odometry could be added instead.
